Decidability of Timed Communicating Automata

We study the reachability problem for networks of timed communicating processes. Each process is a timed automaton communicating with other processes by exchanging messages over unbounded FIFO channels. Messages carry clocks which are checked at the time of transmission and reception with suitable timing constraints. Each automaton can only access its set of local clocks and message clocks of sent/received messages. Time is dense and all clocks evolve at the same rate. Our main contribution is a complete characterisation of decidable and undecidable communication topologies generalising and unifying previous work. From a technical point of view, we use quantifier elimination and a reduction to counter automata with registers.

==> fig_K.tex <==

%\begin{figure}
\begin{wrapfigure}{r}{0.4\textwidth}
	\vspace{-2ex}
	\centering
	\includegraphics[scale=1]{./imgs/fig_K.ai}
	\caption{Cyclic order $K(a, b, c)$.}
	\label{fig:K}
	\vspace{-2ex}
\end{wrapfigure}
%\end{figure}



==> fig_wrapped.tex <==

%\begin{figure}
\begin{wrapfigure}{r}{0.35\textwidth}
%	\vspace{-5ex}
	\centering
	%$\quad$
	\includegraphics[scale=1]{./imgs/fig_wrapping.ai}
	\caption{Fractional wrapping.}
	\label{fig:wrapped}
	\vspace{-10ex}
\end{wrapfigure}
%\end{figure}



==> scratch.tex <==

\section{Scratch section}

\ignore{
\subsection{Remove modulo constraints}

As a preliminary step, we observe that thanks to fractional clocks,
we can remove modulo constraints from integral clocks.
%
We assume \wlg that all modular constraints are over the same modulus $m$.
%
The \tca $\A_p$ will remember in its control states
the modulo equivalence class $\lambda(x_p)$ for every of its integral clocks $(x_p : \N) \in X_p$
in such a way that modular local constraints of the form $x_p - y_p \eqv m k$
can be resolved to be $\true$ or $\false$ just by looking at $\lambda(x_p) - \lambda(y_p) \eqv m k$.
%
Channel constraints are treated in a similar way.
Assume $p$ wants to execute $\sndop m q {\psimod^p \wedge \psi^p}$ where $\psi^p$ does not contain modular constraints.
%
For every integral channel clock $(x_{pq} : \N) \in X_{pq}$,
process $p$ will guess and send to $q$ its modulo class $\lambda(x_{pq})$
by executing $\sndop {\tuple {m, \lambda}} q {\widetilde\psimod^p \wedge \psi^p}$
where $\widetilde\psimod^p$ is obtained by replacing $x_{pq} - y_p \eqv m k$ are directly checked as $\lambda(x_{pq}) - \lambda(y_p) \eqv m k$.


\subsection{Classical and fractional constraints}

Now that there are no modulo constraints,
we transform the remaining integral inequality constraints
into classical and fractional constraints.

}

\subsection{Reduction to a counter machine with registers}

%A \stca is \emph{send-copy} if for every channel $pq \in C$ its set of clocks is of the form
%${X_{pq} = \setof {x_{pq}} {x_p \in X_p}}$, i.e., there is a channel clock for every local clock of $p$,
%and all send operations of $p$ are of the form $\sndop m q {\copyc p q}$, where
%
%\begin{align}
%	\label{eq:send:copy}
%	\copyc p q \equiv \bigwedge_{x_p \in X_p} x_{pq} = x_p.
%\end{align}

Steps:
%
\begin{enumerate}
	
	\item Remove integer diagonal constraints on local clocks (standard).
	
	\item Desynchronised semantics: local clocks can evolve freely as long as for every channel $pq \in C$,
	$x_p^0 \leq x_q^0$, where $x_p^0 \in X_p$ is a local clock which is never reset.
	In this way we can ensure causality between send and receive operations.
	
	\item The desynchronised semantics is implemented by a (untimed) register automaton 
	The amount of desynchronisation is book-kept in a non-negative integer counter $c_{pq}$.
	Whenever $p$ elapses one time unit, $c_{pq}$ is decremented,
	and whenever $q$ elapses one time unit, $c_{pq}$ is incremented.
	
	\item Classical clocks are abstracted by their unary class.
	This suffices since there are no diagonal constraints.
	
	\item Handshaking semantics: Send and receive operations are executed together, atomically, like in handshaking communication.
	This removes the channels and does not lose runs in the desynch semantics.
	%
	Consider a send/receive pair $\sndop m q {\hat x_{pq} = 0}/\rcvop m p {\hat x_{pq} = \hat x_q}$.
	%
	We check $c_{pq} \approx \hat x_q$, i.e.,
	that the counter $c_{pq}$ has the same unary class as $\hat x_q$.
	%
	This suffices since only the unary class of $\hat x_q$ counts in (non-diagonal) classical local constraints of $q$.	
	
	\item
	%
	A receive operation of the form $\rcvop m p \psi$ where $\psi$ contain constraints
	%
	\begin{align*}
		\floor {x_{pq}} - \floor {y_q} &\leq k, \\
		\floor {x_{pq}} - \floor {y_q} &\eqv l k, \\
		\fract {x_{pq}} - \fract {y_q} &\leq 0.
	\end{align*}
	%
	Thanks to send-copy, $x_{pq} = x_p$,
	and due to the desynchronisation,
	the value of channel clock $x_{pq}$ must be increased by $x_q^0 - x_p^0$, obtaining constraints
	\begin{align*}
		\floor {x_p + x_q^0 - x_p^0} - \floor {y_q} &\leq k, \\
		\floor {x_p + x_q^0 - x_p^0} - \floor {y_q} &\eqv l k, \\
		\fract {x_p + x_q^0 - x_p^0} - \fract {y_q} &\leq 0.
	\end{align*}

\ignore{
	
	Time elapse of $p$ is simulated by the constraint
	%
	\begin{align*}
		\elapsec p \ \equiv\ \bigwedge_{q \neq p} \next{\hat x_q^0} = \hat x_q^0 \wedge \bigwedge_{q, x_q} \hat x_q' = \hat x_q.
	\end{align*}
	%
	A reset operation $\resetop Y$ of $p$ is simulated by the constraint
	%
	\begin{align*}
		\resetc p Y \ \equiv\ \bigwedge_q \next{\hat x_q^0} = \hat x_q^0 \wedge
			\bigwedge_{x_p \in Y} \hat x_p' = \hat x_p^0 \wedge
			\bigwedge_{x_p \not\in Y} \hat x_p' = \hat x_p \wedge
			\bigwedge_{q \neq p, x_q} \hat x_q' = \hat x_q.
	\end{align*}
	
}
\end{enumerate}
